Characterizing Metastable Faults and Failures

Metastable failures are hard to detect, prevent, and mitigate. During a metastable failure, a system exhibits self-sustaining bad behavior even in the absence of adversarial conditions. Prior work focuses on symptoms and has portrayed metastable failures as instances of self-sustaining overload. This characterization leaves the underlying failure causes and dynamics unknown, and does not account for metastable failures that do not manifest as overload. We present the first causal characterization of metastable failures by identifying their origin in metastable faults, i.e., structural destabilizing cycles of interaction among systems components that, in isolation, are stabilizing. Metastable failures arise when scheduling decisions let these destabilizing interactions gain the upper hand over the individual components' stabilizing tendencies. We then derive a methodology to predict metastable failures, and to build metastable-fault-tolerant (MFT) systems. We apply our methodology to three case studies, showcasing the generality of our results.

==> composition.tex <==
\section{Metastability and Composition}

==> detection.tex <==
\section{Detecting Metastability}\label{sec: detection}

==> landscape.tex <==
\section{The Landscape}
\subsection{Related Work}

==> practical.tex <==
\section{Practical Insights}\label{sec:practical}
\begin{itemize}
    \item Your system should occasionally shake itself in order to solve the bootstrapping problem.
    It should also be careful when its recovery actions are firing; it should ``slow down'' some parts so that it can drive safely towards its context.
    Perhaps we can demonstrate this with an implementation.

    \item Recovery requires synchronization.

    \item The microservice paradigm exacerbates metastability, for two reasons: ($i$) we are composing things with a higher intensity, and ($ii$) the components are usually designed in isolation.
    In fact, they are encouraged to be designed in isolation, as it speeds up the development pipeline and leads to higher modularity.
\end{itemize}

==> runtime.tex <==
\section{Avoiding Metastability at Runtime}
When your load increases, you should slow down, because you might be driving the system over the cliff for all that you know.
Slowing down gives the system enough time to weather a sudden trigger by having a higher chance of operating based on the recovery interaction blueprint, after which it can go back to the normal interaction blueprint.
The closer you get to your capacity, the slower you should become.
Modern systems do the opposite: the closer they get to the edge of the cliff, the faster they drive.
The question, of course, is how fast you should slow down.
Linear, quadratic, or something else?

A way to infer that something is wrong is by noticing increased ``recovery'' activity in the system.
The potential energy is leaking as kinetic energy.

Here are some demonstrations using our case studies.
Assume that we do not know how these systems are metastable, and we just have an intuitive notion of load for each component.

\subsection{Cache Metastability}
A figure showing the sensitivity of the runoff timer value to the input load intensity.
The higher the load, the higher the timeout.
Show that even a simple, naively adaptive fix helps with metastability.

\subsection{Registry-Coordinator}
A figure showing the sensitivity of the runoff pong timer and the lookup timer to the number of crashes in a trigger.
The higher the ``load'' (the number of crashes), the higher the timers.
Show that even a simple, naively adaptive fix helps with metastability.

Show that, if the system has received a number of crashes, even the timing of healing the crashes is important.
This highlights the importance of ordering between critical events.
You should heal the crash at the right time.
Of course, for this example we need the system that is prone to metastability, not the one that is not metastable by design.

==> solving.tex <==
\section{Solving Metastability}\label{sec: solving}
